Learning Emergent Random Access Protocol for LEO Satellite Networks

A mega-constellation of low-altitude earth orbit (LEO) satellites (SATs) are envisaged to provide a global coverage SAT network in beyond fifth-generation (5G) cellular systems. LEO SAT networks exhibit extremely long link distances of many users under time-varying SAT network topology. This makes existing multiple access protocols, such as random access channel (RACH) based cellular protocol designed for fixed terrestrial network topology, ill-suited. To overcome this issue, in this paper, we propose a novel grant-free random access solution for LEO SAT networks, dubbed emergent random access channel protocol (eRACH). In stark contrast to existing model-based and standardized protocols, eRACH is a model-free approach that emerges through interaction with the non-stationary network environment, using multi-agent deep reinforcement learning (MADRL). Furthermore, by exploiting known SAT orbiting patterns, eRACH does not require central coordination or additional communication across users, while training convergence is stabilized through the regular orbiting patterns. Compared to RACH, we show from various simulations that our proposed eRACH yields 54.6% higher average network throughput with around two times lower average access delay while achieving 0.989 Jain's fairness index.

==> Table/Table_Notation.tex <==
\begin{tabular} {l l}
    % \centering
	%\begin{tabular} {P{1.2cm} P{0.001cm} P{0.001cm} P{0.001cm} P{0.001cm}P{0.001cm} P{0.001cm}}
	\toprule[1pt]
	\textbf{Definition} & \textbf{Notation} \\
% 	Location of UT & $\mathbf{q}_{j}=[0,0,0]^T$ \\  
% 	Location of Dst & $\mathbf{q}_{\mathcal{D}}=[4000,4000,0]^T$ \\
	\midrule
	Altitude of SAT & $H_{\mathrm{L}}=550$ {[}km{]} (from \cite{Starlink}) \\ 
	Velocity (Speed) of SAT1 ($k=1$) & $\mathbf{v}^{1}_{\mathrm{L}, \mathrm{I}}=[0, 7590, 0]^T$ ($7590$ {[}m/s{]}) \\
	Velocity of SAT2 ($k=2$) & $\mathbf{v}^{2}_{\mathrm{L}, \mathrm{I}}=[0, -7590, 0]^T$\\
	Radius of an orbit & $r_{\mathrm{E}} = 6921$ {[}km{]} \\ 
	Circumference of an orbital lane & $c_{\mathrm{E}} = 43486$ {[}km{]} \\ 
	Number of SATs per orbital lane & $I = 22$ \\ 
	Inter-SAT distance & $1977$ {[}km{]}  \\
	Number of UT & $J = 5$ \\
% 	Length an orbital line segment & $c_{\mathrm{C}} = 6000$ {[}km{]} \\ 
% 	Number of SATs per orbital line segment & $I' = 3$ \\ 
	\midrule
	Bandwidth & $B = 10^{8}$ {[}Hz{]} \\   
	Reference SNR ($d=1$ {[}m{]}) & $\gamma_{0} = 10^{11}$ \\ 
    Path loss exponent & $\Tilde{\alpha} = 2.1$    \\
    Parameter for LoS probability & $C=10$, $D=0.6$ \\
    Attenuation factor & $\kappa = 0.2$ \\
	\midrule
% 	Time step size & $\delta_t = \delta_{\mathrm{A}} + \delta_{\mathrm{D}}$  \\
	Random access duration & $\delta_{\mathrm{A}} = 10$ {[}ms{]} \\
	Data transmission duration & $\delta_{\mathrm{D}} = 90$ {[}ms{]}   \\
	Preamble signatures for each SAT & $P = 2 - 54$ \\
	Number of time slots per episode & $N=2604$ \\
% 	Altitude of UAV & $H_{\mathrm{U}}=50$ {[}km{]} (from \cite{Intro_4}) \\
% 	Maximum acceleration of UAV & $A_{\mathrm{max}} = 5$ [m/s$^2$] \\
% 	Discretization level for $a_{j}^{\mathcal{A}}[n]$ & $D = 5$ \\
% 	\midrule
% 	\midrule
% 	Learning rate, Discount factor & $10^{-4}$, 0.995 \\ 
% 	Batch size, \# of iterations/update & 505, 505 \\ 
% 	\# of iterations/episode & 101 \\ 
% 	Training iterations of episode & 5000 \\
	\bottomrule[1pt]
\end{tabular}

